From Micro to Macro: Uncovering and Predicting Information Cascading Process with Behavioral Dynamics

Cascades are ubiquitous in various network environments. How to predict these cascades is highly nontrivial in several vital applications, such as viral marketing, epidemic prevention and traffic management. Most previous works mainly focus on predicting the final cascade sizes. As cascades are typical dynamic processes, it is always interesting and important to predict the cascade size at any time, or predict the time when a cascade will reach a certain size (e.g. an threshold for outbreak). In this paper, we unify all these tasks into a fundamental problem: cascading process prediction. That is, given the early stage of a cascade, how to predict its cumulative cascade size of any later time? For such a challenging problem, how to understand the micro mechanism that drives and generates the macro phenomenons (i.e. cascading proceese) is essential. Here we introduce behavioral dynamics as the micro mechanism to describe the dynamic process of a node's neighbors get infected by a cascade after this node get infected (i.e. one-hop subcascades). Through data-driven analysis, we find out the common principles and patterns lying in behavioral dynamics and propose a novel Networked Weibull Regression model for behavioral dynamics modeling. After that we propose a novel method for predicting cascading processes by effectively aggregating behavioral dynamics, and propose a scalable solution to approximate the cascading process with a theoretical guarantee. We extensively evaluate the proposed method on a large scale social network dataset. The results demonstrate that the proposed method can significantly outperform other state-of-the-art baselines in multiple tasks including cascade size prediction, outbreak time prediction and cascading process prediction.

==> exp_dataset_description_table.tex <==

\begin{table}
    \begin{tabular}[c]{ c | c | c | c}
        \hline \hline
        Cascade size & Cascade & Cascade size & Cascade \\
        limit & number & limit & number \\
        \hline
        over 20 & 141226 & over 100 & 36135 \\
        over 30 & 104537 & over 200 & 16807 \\
        over 40 & 84476 & over 300 & 11221 \\
        over 50 & 70688 & over 400 & 8349 \\
        over 60 & 60436 & over 500 & 6531 \\
        over 70 & 52298 & over 600 & 5293 \\
        over 80 & 45731 & over 800 & 3862 \\
        over 90 & 40547 & over 1000 & 3064 \\
        \hline
        %Lognormal & $\frac{1}{t\sigma_i\sqrt{2\pi}}e^{-\frac{\left(\ln t-\mu_i\right)^2}{2\sigma_i^2}}$ & $\frac{1}{2} + \frac{1}{2}{erf}\left[\frac{\ln t - \mu_i}{\sqrt{2}\sigma_i}\right]$ & $\frac{\frac{1}{t\sigma_i\sqrt{2\pi}}e^{-\frac{\left(\ln t-\mu_i\right)^2}{2\sigma_i^2}}}{\frac{1}{2} + \frac{1}{2}{erf}\left[\frac{\ln t - \mu_i}{\sqrt{2}\sigma_i}\right]}$ & $0.0670$ \\
        %\hline
    \end{tabular}
    \caption{Dataset information}
    \label{table:dataset_description_table}
\end{table}


==> exp_double_test.tex <==
\begin{figure}[htbg]
    \centering
    \includegraphics[width=0.5\textwidth]{double_test.pdf}

    \hspace{0.0002in}
    \caption{Prediction results of different methods with different observation numbers.}
    \label{fig:double_test}
\end{figure}


==> exp_prediction_window_accuracy.tex <==
%\begin{figure*}[htbg]
%    \centering
%    \includegraphics[width=8in]{same_users_unknown_cascades_size_rmse.pdf}
%	\caption{\textbf{RMSE results}. }
%	\label{fig:exp_rmse}
%\end{figure*}
\begin{figure}[htbg]
    \centering
    \includegraphics[width=0.5\textwidth]{prediction_window_accuracy.pdf}

    \hspace{0.0002in}
    \caption{prediction window accuracy with error rate of the size restricted to $0.25$.}
    \label{fig:prediction_window_accuracy}
\end{figure}


==> pre_example.tex <==
\begin{figure}
	\begin{center}
		\tikzset{
			head/.style = {fill = orange!90!blue, label = center:\textsf{\Large H}},
			tail/.style = {fill = blue!70!yellow, text = black,label = center:\textsf{\Large T}},
			occured/.style = {fill = green!80!red},
			future/.style = {fill = red!80!green}
		}
		\begin{tikzpicture}[
				scale = 1.5, transform shape, thick,
				every node/.style = {draw, circle, minimum size = 5mm},
				grow = down,  % alignment of characters
				level 1/.style = {sibling distance=1cm},
				level 2/.style = {sibling distance=1cm},
				level 3/.style = {sibling distance=1cm},
				level distance = 1.5cm
			]
%			\node[fill = gray!40, shape = rectangle, rounded corners,
%				minimum width = 6cm, font = \sffamily] {Coin flipping}
%			child { node[shape = circle split, draw, line width = 1pt,
%				minimum size = 10mm, inner sep = 0mm, font = \sffamily\large,
%				rotate=30] (Start)
%				{ \rotatebox{-30}{H} \nodepart{lower} \rotatebox{-30}{T}}
%				child {   node [head] (A) {test}
%					child { node [head] (B) {}}
%					child { node [tail] (C) {}}
%				}
%				child {   node [tail] (D) {}
%					child { node [head] (E) {}}
%					child { node [tail] (F) {}}
%				}
%			};
			\node [occured, line width = 1pt, font = \sffamily\large] (p1) {$p_1$}
				child{
					node [occured] (p2) {$p_2$}
						child { node [occured] (p4) {$p_4$} }
						child { node [future] (p6) {$p_6$} }
						child { node [future] (p9) {$p_9$} }
				}
				child{ node [occured] (p3) {$p_3$} }
				child{ node [future] (p5) {$p_5$} }
				child{ node [future] (p7) {$p_7$} }
				child{ node [future] (p8) {$p_8$} };

%			\draw (p1.north east)+(0.1,0.5) -- (p1.south east)+(0.1,-0.5);

			% Labels
			\begin{scope} [nodes = {draw = none}]
%				\path (p1) -- node [near end, left] (e1_2) {$1$} (p2) ;
%				\path (p1) -- node [near end, left] (e1_3) {$3$} (p3) ;
%				\path (p1) -- node [near end, left] (e1_5) {$5$} (p5) ;
%				\path (p1) -- node [near end, left] (e1_7) {$10$} (p7) ;
%				\path (p1) -- node [near end, left] (e1_8) {$12$} (p8) ;
%				\path (p2) -- node [near end, left] (e2_4) {$2$} (p4) ;
%				\path (p2) -- node [near end, left] (e2_6) {$10$} (p6) ;
%				\path (p2) -- node [near end, left] (e2_9) {$12$} (p9) ;
				\begin{scope}
					\node (e1_2) at (p2)[xshift=10pt,yshift=15pt] {$1$};
					\node (e1_3) at (p3)[xshift=5pt,yshift=15pt] {$3$};
					\node (e1_5) at (p5)[xshift=4pt,yshift=15pt] {$5$};
					\node (e1_7) at (p7)[xshift=0pt,yshift=15pt] {$10$};
					\node (e1_8) at (p8)[xshift=-6pt,yshift=15pt] {$12$};
					\node (e2_4) at (p4)[xshift=3pt,yshift=15pt] {$2$};
					\node (e2_6) at (p6)[xshift=6pt,yshift=15pt] {$10$};
					\node (e2_9) at (p9)[xshift=0pt,yshift=15pt] {$12$};
				\end{scope}
				\draw [densely dashed, rounded corners, thin] (e1_2.south west) rectangle (e1_8.north east);
				\draw [rounded corners, thin] (e1_2.south west)+(0.03,0.03) rectangle (e1_3.north east)+(-0.03,-0.03);
				\draw [densely dashed, rounded corners, thin] (e2_4.south west) rectangle (e2_9.north east);
				\draw [rounded corners, thin] (e2_4.south west)+(0.03,0.03) rectangle (e2_4.north east)+(-0.03,-0.03);
				\draw[color=blue, line width=3pt] ($(p1)+(16pt,20pt)$) --node [right] {$t = 4$} ($(p1)+(16pt,-18pt)$) -- ($(p1)+(-16pt,-18pt)$) -- ($(p1)+(-16pt,-61pt)$) -- ($(p1)+(-72pt,-61pt)$) -- ($(p1)+(-72pt,-100pt)$);
			\end{scope}

%			% Labels
%			\begin{scope}[nodes = {draw = none}]
%				\path (Start) -- (A) node [near start, left]  {$0.5$};
%				\path (A)     -- (B) node [near start, left]  {$0.5$};
%				\path (A)     -- (C) node [near start, right] {$0.5$};
%				\path (Start) -- (D) node [near start, right] {$0.5$};
%				\path (D)     -- (E) node [near start, left]  {$0.5$};
%				\path (D)     -- (F) node [near start, right] {$0.5$};
%				\begin{scope}[nodes = {below = 11pt}]
%					\node [name = X] at (B) {$0.25$};
%					\node            at (C) {$0.25$};
%					\node [name = Y] at (E) {$0.25$};
%					\node            at (F) {$0.25$};
%				\end{scope}
%				\draw[densely dashed, rounded corners, thin]
%					(X.south west) rectangle (Y.north east);
%			\end{scope}
		\end{tikzpicture}

	\end{center}
	\caption{
		A cascade example. $p_1$ is root post, the others are retweet posts, and the number above the node indicates the reply time of the post to its parent post. Supposing the query time $t_{limit} = 4$, the green nodes on the left of the blue line refer to the posts appeared in the cascade.
%		Social network, information diffusion network and influencial links:
%		The bottom are user nodes in SN and the top are message nodes in IDN.
%		The dashed lines between these two networks show the mapping function $f$
%		from message to its sender.
%		The arrows in SN show social relations, e.g., user $u_3$ follows user $u_1$.
%		The arrows in IDN show the diffusion, e.g.,
%		message $v_3$ is a retweet of message $v_1$,
%		and message $v_5$ is a retweet of $v_4$.
%		$\edge{v_1,v_3}$ and $\edge{v_4,v_5}$ are influencial links on the IDN,
%		which burst the scale of messages.
%		Thus, $\edge{u_1,u_3}$ is the influencial link on the SN.
	}
	\label{fig:example}
\end{figure}


==> pre_example_proportion.tex <==
\begin{figure}
	\begin{center}
		\epsfig{file=cascade_survival_rate.eps,width=3.6in}
	\end{center}
	\caption{survival rate of survival systems $p_1$ and $p_2$}
	\label{fig:example_proportion}
\end{figure}

